An Accurate Hybrid Delay Model for Multi-Input Gates

In order to facilitate the analysis of timing relations between individual transitions in a signal trace, dynamic digital timing analysis offers a less accurate but much faster alternative to analog simulations of digital circuits. This primarily requires gate delay models that also account for the fact that the input-to-output delay of a particular input transition also depends on the temporal distance to the previous output transitions. In the case of multi-input gates, the delay also experiences variations caused by multi-input switching (MIS) effects, i.e., transitions at different inputs that occur in close temporal proximity. In this paper, we advocate the development of hybrid delay models for CMOS gates obtained by replacing transistors with time-variant resistors. We exemplify our approach by applying it to a NOR gate (and, hence, to the dual NAND gate) and a Muller C gate. We analytically solve the resulting first-order differential equations with non-constant-coefficients, and derive analytic expressions for the resulting MIS gate delays. The resulting formulas not only pave the way to a sound model parametrization procedure, but are also instrumental for implementing fast and efficient digital timing simulation. By comparison with analog simulation data, we show that our models faithfully represent all relevant MIS effects. Using an implementation in the Involution Tool, we demonstrate that our model surpasses the alternative digital delay models for NOR gates known to us in terms of accuracy, with comparably short running times.

==> Latex (ICCAD versions)/common.tex <==
% delay function
\newcommand{\dinv}[1]{d^{-1}(#1)}
\newcommand{\de}{d}
\newcommand{\dup}{\delta_\uparrow}
\newcommand{\ddo}{\delta_\downarrow}
\newcommand{\fup}{f_\uparrow}
\newcommand{\fdo}{f_\downarrow}
\newcommand{\dupD}{\delta^\uparrow}
\newcommand{\ddoD}{\delta^\downarrow}

\newcommand{\dsu}{\delta_S^\uparrow}
\newcommand{\dsd}{\delta_S^\downarrow}
\newcommand{\dmu}{\delta_M^\uparrow}
\newcommand{\dmd}{\delta_M^\downarrow}
\newcommand{\dsud}{\delta_S^{\uparrow/\downarrow}}

\newcommand{\fIO}{f_\downarrow^{10}}
\newcommand{\fOI}{f_\downarrow^{01}}
\newcommand{\fII}{f_\downarrow^{11}}
\newcommand{\fOO}{f_\uparrow^{00}}

\newcommand{\tauOO}{\tau_{\mathit{int}}^{00}}
\newcommand{\tauOI}{\tau_{\mathit{int}}^{01}}
\newcommand{\tauIO}{\tau_{\mathit{int}}^{10}}
\newcommand{\tauII}{\tau_{\mathit{int}}^{11}}

\newcommand{\tauoOO}{\tau_{out}^{00}}
\newcommand{\tauoOI}{\tau_{out}^{01}}
\newcommand{\tauoIO}{\tau_{out}^{10}}
\newcommand{\tauoII}{\tau_{out}^{11}}

%\newcommand{\AOO}{A^{00}}
%\newcommand{\AOI}{A^{01}}
%\newcommand{\AIO}{A^{10}}
%\newcommand{\AII}{A^{11}}

\newcommand{\dft}[2]{\delta_{#1 \rightarrow #2}}
\newcommand{\dftu}[2]{\delta_{#1 \rightarrow #2}^{M}}
\newcommand{\dftl}[2]{\delta_{#1 \rightarrow #2}^{C}}
%--------- for typical fasy logic papers:

\newcommand{\figPath}[1]{figures/#1}

\newcommand{\NOR}{\texttt{NOR}}
\newcommand{\NAND}{\texttt{NAND}}
\newcommand{\GOR}{\texttt{OR}}
\newcommand{\XOR}{\texttt{XOR}}
\newcommand{\AOI}{\texttt{AOI}}
\newcommand{\C}{\texttt{C}}

\newcommand{\dmin}{\delta_{\mathrm{min}}}
\newcommand{\dinfty}{\delta_{\infty}}
\newcommand{\dupinfty}{\delta^\uparrow_\infty}
\newcommand{\ddoinfty}{\delta^\downarrow_\infty}
\newcommand{\ddm}{\textit{DDM}}
\newcommand{\idm}{\textit{IDM}}
\newcommand{\etam}{$\eta$-\textit{model}}
\newcommand{\hspice}{\textit{HSPICE}}
\newcommand{\spice}{\textit{SPICE}}

\newcommand{\Dd}{\Delta \delta}
\newcommand{\DT}{\Delta T}

\newcommand{\dtup}{\Delta t_\uparrow}
\newcommand{\dtdo}{\Delta t_\downarrow}
\newcommand{\tdo}{t_\downarrow}
\newcommand{\tup}{t_\uparrow}
\newcommand{\kdo}{k_\downarrow}
\newcommand{\kup}{k_\uparrow}
\newcommand{\tvth}{t_{vth}}
\newcommand{\ts}{T_{2}}
\newcommand{\ds}{\delta_{2}}
\newcommand{\fud}{f_{\uparrow/\downarrow}}

\newcommand{\vth}{V_{th}}
\newcommand{\vthin}{V_{th}^{in}}
\newcommand{\vthout}{V_{th}^{out}}
\newcommand{\vdd}{V_{DD}}
\newcommand{\gnd}{\textit{GND}}
\newcommand{\vout}{V_{out}}
\newcommand{\vin}{V_{I}}
\newcommand{\dd}{\mathrm{d}}

\newcommand{\vsd}{V_{SD}}
\newcommand{\vds}{V_{DS}}
\newcommand{\vgs}{V_{GS}}
\newcommand{\vsg}{V_{SG}}
\newcommand{\vgd}{V_{GD}}
\newcommand{\vgx}{V_{GX}}
\newcommand{\vdx}{V_{DX}}

\newcommand{\va}{V_{A}}
\newcommand{\vb}{V_{B}}

\newcommand{\vint}{V_{int}}
\newcommand{\cint}{C_{int}}
\newcommand{\iintm}[1]{I_{\mathit{N}}^{#1}}

\newcommand{\cin}{C_{\mathit{in}}}

\newcommand{\cl}{C_{L}}
\newcommand{\cout}{C}

\newcommand{\id}{I_{D}}
\newcommand{\iout}{I_{\mathit{O}}}
\newcommand{\Diout}{\Delta I_{\mathit{out}}}
\newcommand{\inmos}{I_{n}}
\newcommand{\ipmos}{I_{p}}

\newcommand{\tvthup}{t_{th}^\uparrow}
\newcommand{\tvthdo}{t_{th}^\downarrow}

\newcommand{\etp}{\eta^+}
\newcommand{\etm}{\eta^-}

\newcommand{\nmos}{nMOS}
\newcommand{\pmos}{pMOS}
\newcommand{\nandpmos}{n- and pMOS}
\newcommand{\scalen}{S_{n}}
\newcommand{\scalep}{S_{p}}
\newcommand{\vthn}{V_{th,n}}
\newcommand{\vthp}{V_{th,p}}

\newcommand{\st}{(ST)}
\newcommand{\ohm}{(OHM)}
\newcommand{\sat}{(SAT)}

\newcommand{\mystate}[1]{\tikz[overlay]{\node[yshift=3pt, xshift=5pt, circle, draw, line width=1.5pt, inner
    sep=1pt] {\small #1}} \hspace{0.6em}}

\newcommand{\on}{\mbox{\emph{on}}}
\newcommand{\off}{\mbox{\emph{off}}}

%\DeclareMathOperator{\ln}{ln}


==> Latex (ICCAD versions)/mybib.tex <==
% Encoding: UTF-8
@techreport{NP73:spice,
    Author = {Nagel, Laurence W. and Pederson, D.O.},
    Title = {{SPICE} ({S}imulation {P}rogram with {I}ntegrated {C}ircuit {E}mphasis)},
    Institution = {EECS Department, University of California, Berkeley},
    Year = {1973},
    OPTURL = {http://www.eecs.berkeley.edu/Pubs/TechRpts/1973/22871.html},
    Number = {UCB/ERL M382}
}

@ARTICLE{DS90,
author={Deng, A.-C. and Shiau, Y.-C.},
journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
title={Generic linear {RC} delay modeling for digital {CMOS} circuits},
year={1990},
volume={9},
number={4},
pages={367--376},
OPTdoi={10.1109/43.45868},
OPTISSN={0278-0070}
}

@PhdThesis{Ho84:thesis,
  author = 	 {Mark Alan Horowitz},
  title = 	 {Timing Models for {MOS} Circuits},
  school = 	 {Stanford University},
  year = 	 {1984},
  OPTkey = 	 {},
  OPTtype = 	 {},
  OPTaddress = 	 {},
  OPTmonth = 	 {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@ARTICLE{LM84,
author={Tzu-Mu Lin and Mead, C.A.},
journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
title={Signal Delay in General {RC} Networks},
year={1984},
volume={3},
number={4},
pages={331--349},
OPTdoi={10.1109/TCAD.1984.1270090},
OPTISSN={0278-0070}
}

@ARTICLE{PR90,
author={Pillage, L.T. and Rohrer, R.A.},
journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
title={Asymptotic waveform evaluation for timing analysis},
year={1990},
volume={9},
number={4},
pages={352--366},
OPTdoi={10.1109/43.45867},
OPTISSN={0278-0070}
}

@book{Ash08,
author = {Peter J. Ashenden},
title = {The Designer’s Guide to VHDL},
edition = {third},
publisher = {Morgan Kaufmann},
address = {Burlington},
year = 2008
}

@article{BJ83,
author = {Jos\'e C. Barros and Brian W. Johnson},
title = {Equivalence of the Arbiter, the Synchronizer, the Latch, and the
Inertial Delay},
journal = {IEEE Transactions on Computers},
volume = 32,
number = 7,
pages = {603--614},
year = 1983
}

@article{BDJCAVH00,
author = {M. J. Bellido-D{\'{\i}}az
	and J. Juan-Chico
	and A. J. Acosta
	and M. Valencia
	and J. L. Huertas},
title = {Logical Modelling of Delay Degradation Effect in Static {CMOS} Gates},
journal = {IEE Proceedings -- Circuits, Devices, and Systems},
volume = 147,
number = 2,
pages = {107--117},
year = 2000
}

@article{Bra95,
author = {Michael S. Branicky},
title = {Universal Computation and Other Capabilities of Hybrid and Continuous
Dynamical Systems},
journal = {Theoretical Computer Science},
volume = 138,
number = 1,
pages = {67--100},
year = 1995
}

@article{BE92,
author = {Janusz A. Brzozowski and Jo C. Ebergen},
title = {On the Delay-Sensitivity of Gate Networks},
journal = {IEEE Transactions on Computers},
volume = 41,
number = 11,
pages = {1349--1360},
year = 1992
}

@book{Dol00,
author = {Shlomi Dolev},
title = {Self-Stabilization},
publisher = {MIT Press},
address = {Cambridge},
year = 2000
}

@incollection{DFLS11,
author = {D. Dolev and M. F\"ugger and C. Lenzen and U. Schmid},
title = {Fault-Tolerant Algorithms for Tick-Generation in Asynchronous Logic:
Robust Pulse Generation},
booktitle = {Proceeding of the 13th International Symposium on Stabilization,
Safety, and Security of Distributed Systems (SSS)},
editor = {Xavier D\'efago and Franck Petit and Vincent Villain},
series    = {LNCS},
volume    = {6976},
publisher = {Springer},
address = {Heidelberg},
pages = {163--177},
year = 2011
}


@book{DT97,
author = {Michael Drmota and Robert F. Tichy},
title = {Sequences, Discrepancies, and Applications},
publisher = {Springer},
address = {Heidelberg},
year = 1997
}

@incollection{FFS09,
author = {Gottfried Fuchs and Matthias F\"ugger and Andreas Steininger},
title = {On the Threat of Metastability in an Asynchronous Fault- Tolerant
Clock Generation Scheme},
booktitle = {Proceedings of the 15th IEEE International Symposium on
Asynchronous Circuits and Systems (ASYNC)},
publisher = {IEEE Press},
address = {New York City},
pages = {127--136},
year  =2009
}

@article{FS12,
author = {Matthias F\"ugger and Ulrich Schmid},
title = {Reconciling Fault-Tolerant Distributed Computing and Systems-on-Chip},
journal = {Distributed Computing},
volume = 14,
number = 6,
pages = {323--355},
year = 2012
}

@article{GEBC06,
author = {Matthew J. Gadledge and Paul H. Eaton and Joseph M. Benedetto and
Marty Carts and Vivian Zhu and Thomas L. Turflinger},
title = {Digital Device Error Rate Trends in Advanced {CMOS} Technologies},
journal = {IEEE Transactions on Nuclear Science},
volume = 53,
number = 6,
pages = {3466--3471},
year = 2006
}

@book{Kin07,
author = {David J. Kinniment},
title = {Synchronization and Arbitration in Digital Systems},
publisher = {Wiley},
address = {Chichester},
year = 2007
}

@article{Mar77,
author = {Leonard R. Marino},
title = {The Effect of Asynchronous Inputs on Sequential Network Reliability},
journal = {IEEE Transactions on Computers},
volume = 26,
number = 11,
pages = {1082--1090},
year = 1977
}

@article{Mar81,
author = {Leonard R. Marino},
title = {General Theory of Metastable Operation},
journal = {IEEE Transactions on Computers},
volume = 30,
number = 2,
pages = {107--115},
year = 1981
}

@incollection{MA01,
author = {M. Salim Maza and M. Linares Aranda},
title = {Analysis of Clock Distribution Networks in the Presence of Crosstalk
and Groundbounce},
booktitle = {Proceedings of the 8th IEEE International Conference on
Electronics, Circuits, and Systems (ICECS)},
publisher = {IEEE Press},
address = {New York City},
pages = {773--776},
year = 2001
}

@article{MS93,
author = {Michael Mendler and Terry Stroup},
title = {Newtonian Arbiters Cannot Be Proven Correct},
journal = {Formal Methods in System Design},
volume = 3,
number = 3,
pages = {233--257},
year = 1993
}

@article{RCS90,
author = {Fred U. Rosenberger and Charles E. Molnar and Thomas J. Chaney and
Ting-Pien Fang},
title = {Q-Modules: Internally Clocked Delay-Insensitive Modules},
journal = {IEEE Transactions on Computers},
volume = 37,
number = 9,
pages = {1005--1018},
year = 1988
}

@article{Sch93,
author = {Johannes Schoissengeier},
title = {The discrepancy of $(n\alpha)_{n\geq1}$},
journal = {Mathematische Annalen},
volume = 296,
number = 1,
pages = {529--545},
year = 1993
}

@article{Sut89,
author = {Ivan E. Sutherland},
title = {Micropipelines},
journal = {Communications of the ACM},
volume = 32,
number = 6,
pages = {720--738},
year = 1989
}

@article{Ung71,
author = {Stephen H. Unger},
title = {Asynchronous Sequential Switching Circuits with Unrestricted Input
Changes},
journal = {IEEE Transaction on Computers},
volume = 20,
number = 12,
pages = {1437--1444},
year = 1971
}

@book{BJV06,
author = {Manuel J. Bellido-D{\'{\i}}az and Jorge Juan-Chico and Manuel Valencia},
title = {Logic-Timing Simulation and
the Degradation Delay Model},
publisher = {Imperial College Press},
address = {London},
year = 2006
}

@article{Con03,
author = {Cristian Constantinescu},
title = {Trends and Challenges in {VLSI} Circuit Reliability},
journal = {IEEE Micro},
volume = 23,
number = 4,
pages = {14--19},
year = 2003
}

@incollection{FNS13,
author = {Matthias F\"ugger and Thomas Nowak and Ulrich Schmid},
title = {Unfaithful Glitch Propagation in Existing Binary Circuit Models},
booktitle = {Proceedings of the 19th IEEE International Symposium on
Asynchronous Circuits and Systems (ASYNC)},
publisher = {IEEE Press},
address = {New York City},
pages = {191--199},
year = 2013
}

@MISC{Syn05:CCS,
author={Synopsis},
title={{CCS} Timing},
howpublished={Technical white paper v2.0, 2006},
}


@ARTICLE{Naj94,
author={Najm, F.N.},
journal={Very Large Scale Integration (VLSI) Systems, IEEE Transactions on},
title={A survey of power estimation techniques in {VLSI} circuits},
year={1994},
volume={2},
number={4},
pages={446-455},
doi={10.1109/92.335013},
ISSN={1063-8210}
}
@inproceedings{FB95,
 author = {Favalli, M. and Benini, L.},
 title = {Analysis of glitch power dissipation in {CMOS} {IC}s},
 booktitle = {Proceedings of the 1995 international symposium on Low power desig
n},
 series = {ISLPED '95},
 year = {1995},
 isbn = {0-89791-744-8},
 location = {Dana Point, California, USA},
 pages = {123--128},
 numpages = {6},
 doi = {10.1145/224081.224103},
 acmid = {224103},
 publisher = {ACM},
 address = {New York, NY, USA},
}
@inproceedings{FNS13:ASYNC,
  author    = {Matthias F{\"u}gger and Thomas Nowak and Ulrich Schmid},
  title     = {Unfaithful Glitch Propagation in Existing Binary Circuit Models},
  booktitle = {Proceedings 19th IEEE International Symposium on Asynchronous Circuits and Systems (ASYNC'13)},
  year      = {2013},
  pages = {191-199},
ee        = {http://doi.ieeecomputersociety.org/10.1109/ASYNC.2013.9},
publisher = {IEEE Computer Society},
}

@ARTICLE{FNS16:ToC,
author={Matthias F\"ugger and Thomas Nowak and Ulrich Schmid},
journal={IEEE Transactions on Computers},
title={Unfaithful Glitch Propagation in Existing Binary Circuit Models},
year={2016},
volume={65},
number={3},
pages={964-978},
keywords={Analytical models;Computational modeling;Delays;Integrated circuit mod
eling;Inverters;Logic gates;Circuit models;binary models;glitch propagation;mode
ling issues},
doi={10.1109/TC.2015.2435791},
ISSN={0018-9340},
month={March},
}

@incollection{JBRA00,
year={2000},
isbn={978-3-540-41068-3},
booktitle={Integrated Circuit Design},
series={LNCS 1918},
doi={10.1007/3-540-45373-3_15},
title={Degradation Delay Model Extension to {CMOS} Gates},
publisher={Springer},
author={Juan-Chico, Jorge and Bellido, Manuel J. and Ruiz-de-Clavijo, Paulino and Acosta, Antonio J. and Valencia, Manuel},
pages={149-158},
language={English}
}

@incollection{MJBR02,
year={2002},
isbn={978-3-540-44143-4},
booktitle={Integrated Circuit Design},
series={LNCS 2451},
doi={10.1007/3-540-45716-X_48},
title={Characterization of Normal Propagation Delay for Delay Degradation Model {(DDM)}},
publisher={Springer},
author={Millan, Alejandro and Juan, Jorge and Bellido, Manuel J. and Ruiz-de-Clavijo, Paulino and Guerrero, David},
pages={477-486},
language={English}
}

@article{HSDZ12:ToNS,
  author =       "Michael Hofbauer and Kurt Schweiger and Horst Dietrich and Horst Zimmermann and Kay-Obbe Voss and Bruno Merk and Ulrich Schmid and Andreas Steininger",
  title =        "Pulse Shape Measurements by On-chip Sense Amplifiers of Single
 Event Transients Propagating through a 90 nm Bulk {CMOS} Inverter Chain",
  journal =      "IEEE Transactions on Nuclear Science",
  year =         "2012",
  month = dec,
  volume = 59,
  number = 6,
  pages = {2778-2784},
}

@manual{Syn:CCSM,
organization={Synopsis Inc.},
title={{CCS} Timing Library Characterization Guidelines},
month={October},
year={2016},
note={Version 3.4}
}

@manual{Cad:ECSM,
organization={Cadence Design Systems},
title={Effective Current Source Model {(ECSM)} Timing and Power Specification},
month={January},
year={2015},
note={Version 2.1.2}
}

@inproceedings{NFNS15:GLSVLSI,
 author = {Najvirt, Robert and Schmid, Ulrich and Hofbauer, Michael and F\"{u}gger, Matthias and Nowak, Thomas and Schweiger, Kurt},
 title = {Experimental Validation of a Faithful Binary Circuit Model},
 booktitle = {Proceedings of the 25th Edition on Great Lakes Symposium on VLSI},
 series = {GLSVLSI '15},
 year = {2015},
 isbn = {978-1-4503-3474-7},
 location = {Pittsburgh, Pennsylvania, USA},
 pages = {355--360},
 numpages = {6},
 url = {http://doi.acm.org/10.1145/2742060.2742081},
 doi = {10.1145/2742060.2742081},
 acmid = {2742081},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {binary circuit models, delay models, vlsi},
} 


@book{BJV:DDM05,
author = {Bellido, Manuel J and Juan, Jorge and Valencia, Manuel},
title = {Logic-Timing Simulation and the Degradation Delay Model},
publisher = {Imperial College},
year = {2005},
doi = {10.1142/p411},
address = {},
edition   = {},
URL = {https://www.worldscientific.com/doi/abs/10.1142/p411},
eprint = {https://www.worldscientific.com/doi/pdf/10.1142/p411}
}

@inproceedings{FNNS15:DATE,
 author = {F\"{u}gger, Matthias and Najvirt, Robert and Nowak, Thomas and Schmid, Ulrich},
 title = {Towards Binary Circuit Models That Faithfully Capture Physical Solvability},
 booktitle = {Proceedings of the 2015 Design, Automation \& Test in Europe Conference \& Exhibition},
 series = {DATE '15},
 year = {2015},
 pages = {1455--1460},
 publisher = {EDA Consortium},
 address = {San Jose, CA, USA},
}

@INPROCEEDINGS{FMNNS18:DATE,
author={M. F{\"u}gger and J. Maier and R. Najvirt and T. Nowak and U. Schmid},
booktitle={2018 Design, Automation Test in Europe Conference Exhibition (DATE)},
title={A faithful binary circuit model with adversarial noise},
year={2018},
volume={},
number={},
pages={1327-1332},
keywords={delay circuits;digital circuits;formal verification;network synthesis;IEEE TC 2016;accurate delay models;adversarial noise;delay functions;delay shifts;deterministic delay function;digital circuits;dynamic timing analysis;even adversarial;faithful binary circuit model;faithful digital circuit models;formal verification;generalized involution model;involution delays;mathematical involutions;nondeterministic delay variations;pure inertial delays;random adversarial;static timing analysis;Analytical models;Delays;Digital circuits;Integrated circuit modeling;Logic gates;Tools},
doi={10.23919/DATE.2018.8342219},
ISSN={},
month={March},
url={https://ieeexplore.ieee.org/document/8342219/}
}

@BOOK{arora1993,
author = {Arora, Narain},
title = {MOSFET models for VLSI circuit simulation; theory and practice},
series = {Computational microelectronics},
year = {1993},
address = {Wien [u.a.]},
publisher = {Springer},
ISBN = {3-211-82395-6; 0-387-82395-6},
keywords = {MOS-FET ; VLSI; Freies Schlagwort: MOS-FET - VLSI; Metal oxide
semiconductor field-effect transistors ; Mathematical models; Integrated
circuits ; Very large scale integration ; Mathematical models; Integrated
circuits ; Very large scale integration ; Computer simulation},
}

@techreport{M17:TR,
key = {2017},
    author = {Maier, J{\"u}rgen},
    title = {Modeling the CMOS Inverter using Hybrid Systems},
    institution = {E182 - Institut f{\"u}r Technische Informatik; Technische Universit{\"a}t Wien},
    year = {2017},
    number = {TUW-259633},
    url = {http://publik.tuwien.ac.at/files/publik\_259633.pdf}
}

@book {Sze,
title = {Physics of Semiconductor Devices},
author = {Sze, S.M. and Ng, Kwok K.},
publisher = {John Wiley \& Sons, Inc.},
isbn = {9780471143239},
year = {2007},
edition = {third}
}

@MISC{Mathematica,
title={Wolfram Mathematica},
howpublished={\url{https://www.wolfram.com/mathematica/}},
note={Accessed: 2018-12-07}
}


@INPROCEEDINGS{JBAB93,
    author = {Juan-Chico Bellido Acosta and J. Juan-chico and M. J. Bellido and A. J. Acosta and A. Bar
riga and M. Valencia and Sevilla Centro and Nacional Microelectrónica},
    title = {Delay degradation effect in submicronic {CMOS} inverters},
    booktitle = {Proc. FODO'93},
    year = {1997},
    pages = {215--224},
    publisher = {Springer}
}

@inproceedings{Nangate15,
 author = {Martins, Mayler and Matos, Jody Maick and Ribas, Renato P. and Reis, Andr{\'e} and Schlinker, Guilherme and Rech, Lucio and Michelsen, Jens},
 title = {Open Cell Library in 15Nm FreePDK Technology},
 booktitle = {Proceedings of the 2015 Symposium on International Symposium on Physical Design},
 series = {ISPD '15},
 year = {2015},
 isbn = {978-1-4503-3399-3},
 location = {Monterey, California, USA},
 pages = {171--178},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/2717764.2717783},
 doi = {10.1145/2717764.2717783},
 acmid = {2717783},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@INPROCEEDINGS{CharlieEffect,
author={A. J. Winstanley and A. Garivier and M. R. Greenstreet},
booktitle={Proceedings of the 8th International Symposium on Asynchronous Circuits and Systems (ASYNC)},
title={{An Event Spacing Experiment}},
year={2002},
pages={47-56},
keywords={asynchronous circuits;delays;hysteresis;pipeline
processing;timing;Charlie Diagrams;attractors;evenly spaced behaviours;event
spacing experiment;hysteresis;phase transitions;self-timed pipelines;self-timed
rings;standard bounded delay models;timing analysis;Clocks;Delay;Distributed
processing;Fabrication;Hysteresis;Pipelines;Semiconductor device
modeling;Testing;Throughput;Timing}, 
doi={10.1109/ASYNC.2002.1000295},
ISSN={1522-8681},
month={April},}

@book{strang2014differential,
  title={Differential equations and linear algebra},
  author={Strang, Gilbert},
  year={2014},
  publisher={Wellesley-Cambridge Press Wellesley}
}

@INPROCEEDINGS{EFS98:ASYNC,
  author={J. C. {Ebergen} and S. {Fairbanks} and I. E. {Sutherland}},
  booktitle={Proceedings Fourth International Symposium on Advanced Research in Asynchronous Circuits and Systems (ASYNC'98)}, 
  title={Predicting performance of micropipelines using Charlie diagrams}, 
  year={1998},
  volume={},
  number={},
  pages={238-246},
  doi={10.1109/ASYNC.1998.666509}}

@ARTICLE{FNNS19:TCAD,
author={M. {Függer} and R. {Najvirt} and T. {Nowak} and U. {Schmid}},
journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
title={A Faithful Binary Circuit Model},
year={2020},
volume={39},
number={10},
pages={2784-2797},
keywords={Binary circuit models;glitch propagation},
doi={10.1109/TCAD.2019.2937748},
ISSN={0278-0070},}
%month={October},}

@article{OMFS20:INTEGRATION,
title = "The Involution Tool for Accurate Digital Timing and Power Analysis",
journal = "Integration",
volume = "76",
pages = "87 - 98",
year = "2021",
issn = "0167-9260",
doi = "https://doi.org/10.1016/j.vlsi.2020.09.007",
author = "Daniel Öhlinger and Jürgen Maier and Matthias Függer and Ulrich Schmid",
keywords = "Digital timing simulation, Design tools, Delay models, Pulse degradation, Glitch propagation",
}

@Manual{MSIM:FLI,
  title  = {Foreign Language Interface Manual},
  author = {{Mentor Graphics Corporation}},
  note   = {{Software Version 10.5c}},
  year   = {2016},
}

@INPROCEEDINGS{CGB01:DAC,
author={Liang-Chi Chen and S. K. Gupta and M. A. Breuer},
booktitle={Proceedings of the 38th Design Automation Conference (IEEE
Cat. No.01CH37232)}, 
title={A new gate delay model for simultaneous switching and its applications},
year={2001},
pages={289-294},
keywords={automatic test pattern generation;combinational circuits;delays;logic
gates;logic testing;timing;delay phenomena;gate delay model;incremental timing
refinement;simultaneous switching;static timing analysis;targeted delay
phenomena;timing-based ATPG;to-controlling transitions;transition
times;Accuracy;Automatic test pattern generation;Benchmark
testing;Circuits;Computational modeling;Delay effects;Performance
analysis;Permission;Table lookup;Timing}, 
doi={10.1109/DAC.2001.156153},
ISSN={0738-100X},
month={},}

@article{SRC15:TDAE,
 author = {Subramaniam, Anupama R. and Roveda, Janet and Cao, Yu},
 title = {A Finite-Point Method for Efficient Gate Characterization Under
 Multiple Input Switching},
 journal = {ACM Trans. Des. Autom. Electron. Syst.},
 issue_date = {November 2015},
 volume = {21},
 number = {1},
 month = dec,
 year = {2015},
 issn = {1084-4309},
 pages = {10:1--10:25},
 articleno = {10},
 numpages = {25},
 url = {http://doi.acm.org/10.1145/2778970},
 doi = {10.1145/2778970},
 acmid = {2778970},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Characterization, design flow, finite point method, flow, logic,
 multiple input switching, performance verification, standard cell
 characterization}, 
} 


@INPROCEEDINGS{SKJPC09:ISOCC,
author={J. Shin and J. Kim and N. Jang and E. Park and Y. Choi},
booktitle={2009 International SoC Design Conference (ISOCC)},
title={A gate delay model considering temporal proximity of Multiple Input
Switching}, 
year={2009},
pages={577-580},
keywords={delay circuits;integrated circuit modelling;radial basis function
networks;accurate gate delay;delay variation;gate delay model;multiple input
switching;radial basis function;temporal proximity;Capacitance;Circuit
analysis;Clocks;Computer science;Delay effects;Delay
estimation;Frequency;Libraries;MOSFETs;Timing;cell characterization;delay
model;multiple input switching;proximity;temporal}, 
doi={10.1109/SOCDC.2009.5423815},
month={Nov},}

@INPROCEEDINGS{SC06:DATE,
author={J. Sridharan and T. Chen},
booktitle={Proceedings of the Design Automation Test in Europe Conference},
title={Modeling multiple input switching of CMOS gates in DSM technology using
HDMR}, 
year={2006},
volume={1},
pages={6 pp.-},
keywords={CMOS logic circuits;delays;integrated circuit modelling;logic
gates;CMOS gates;DSM chips;SPICE;gate level delays;high dimensional model
representation method;logic gate;multiple input switching modeling;relative
signal arrival times;static timing analysis;CMOS logic circuits;CMOS
technology;Clocks;Delay effects;Delay systems;Logic gates;Semiconductor device
modeling;Signal analysis;Signal processing;Timing}, 
doi={10.1109/DATE.2006.244008},
ISSN={1530-1591},
month={March},}

@ARTICLE{RS21:TCAD,
  author={Shashank Ram, O. V. S. and Saurabh, Sneh},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems}, 
  title={Modeling Multiple-Input Switching in Timing Analysis Using Machine Learning}, 
  year={2021},
  volume={40},
  number={4},
  pages={723-734},
  doi={10.1109/TCAD.2020.3009624}}

@article{Melcher92:MAM,
title = "Multiple input transitions in CMOS gates",
journal = "Microprocessing and Microprogramming",
volume = "35",
number = "1",
pages = "683 - 690",
year = "1992",
note = "Software and Hardware: Specification and Design",
issn = "0165-6074",
doi = "http://dx.doi.org/10.1016/0165-6074(92)90387-M",
url = "http://www.sciencedirect.com/science/article/pii/016560749290387M",
author = "Elmar Melcher and Wolfgang Röthig and Michel Dana",
}

@INPROCEEDINGS{AB06:SST,
author={N. Abdallah and P. Bazargan-Sabet},
booktitle={2006 Proceeding of the Thirty-Eighth Southeastern Symposium on System Theory},
title={Modeling the Effects of Input Slew Rate and Temporal Proximity of Input
Transitions in Event-Driven Simulation}, 
year={2006},
pages={185-189},
keywords={MOS digital integrated circuits;circuit simulation;MOS digital
circuits;event-driven selective-trace paradigm;input slew rate;input
transitions;switch-level timing simulation;temporal proximity;Accuracy;Circuit
simulation;Digital circuits;Discrete event simulation;Predictive
models;Shape;Switching circuits;Timing;Very large scale integration;Voltage}, 
doi={10.1109/SSST.2006.1619069},
ISSN={0094-2898},
month={March},}

@INPROCEEDINGS{SHWW14:ICCAD,
  author={Schneider, Eric and Holst, Stefan and Wen, Xiaoqing and Wunderlich, Hans-Joachim},
  booktitle={2014 IEEE/ACM International Conference on Computer-Aided Design (ICCAD)}, 
  title={Data-parallel simulation for fast and accurate timing validation of CMOS circuits}, 
  year={2014},
  volume={},
  number={},
  pages={17-23},
  doi={10.1109/ICCAD.2014.7001324}}


@inproceedings{FMOS22:DATE,
  author    = {Arman Ferdowsi and
               J{\"{u}}rgen Maier and
               Daniel {\"{O}}hlinger and
               Ulrich Schmid},
  title     = {A Simple Hybrid Model for Accurate Delay Modeling of a Multi-Inpu
t
               Gate},
booktitle = {Proceedings of the 2022 Design, Automation \& Test in Europe Confer
ence \& Exhibition},
 series = {DATE '22},
  year      = {2022},
}


@misc{FMOS21:arxiv,
      title={{A Simply Hybrid Model for Accurate Delay Modeling of a Multi-Input Gate}},
      author={Arman Ferdowsi and J\"urgen Maier and Daniel \"Ohlinger and Ulrich Schmid},
      year={2021},
      note={TechRxiv e-prints, to appear in Proc. DATE'22},
      doi={10.36227/techrxiv.17054906},
      url = {http://doi.acm.org/10.36227/techrxiv.17054906},
}

@ARTICLE{ShichmanHodges,
author={H. {Shichman} and D. A. {Hodges}},
journal={IEEE Journal of Solid-State Circuits},
title={Modeling and simulation of insulated-gate field-effect transistor switching circuits},
year={1968},
volume={3},
number={3},
pages={285-289},
keywords={computer-aided circuit analysis;Computer-aided circuit
                  analysis;Circuit simulation;Insulation;FETs;Switching
                  circuits;Computational modeling;Equivalent circuits;Computer
                  aided analysis;Computer simulation;Application
                  software;Application specific integrated circuits},
doi={10.1109/JSSC.1968.1049902},
ISSN={0018-9200},
month={Sep.},}


@Comment{jabref-meta: databaseType:bibtex;}

%url = "http://www.sciencedirect.com/science/article/pii/S0167926020302777",

@article{BVMRRVB19,
author = {Bouvier, Maxence and Valentian, Alexandre and Mesquida, Thomas and Rummens, Francois and Reyboz, Marina and Vianello, Elisa and Beigne, Edith},
title = {Spiking Neural Networks Hardware Implementations and Challenges: A Survey},
year = {2019},
issue_date = {April 2019},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {15},
number = {2},
issn = {1550-4832},
url = {https://doi.org/10.1145/3304103},
doi = {10.1145/3304103},
abstract = {Neuromorphic computing is henceforth a major research field for both academic and industrial actors. As opposed to Von Neumann machines, brain-inspired processors aim at bringing closer the memory and the computational elements to efficiently evaluate machine learning algorithms. Recently, spiking neural networks, a generation of cognitive algorithms employing computational primitives mimicking neuron and synapse operational principles, have become an important part of deep learning. They are expected to improve the computational performance and efficiency of neural networks, but they are best suited for hardware able to support their temporal dynamics. In this survey, we present the state of the art of hardware implementations of spiking neural networks and the current trends in algorithm elaboration from model selection to training mechanisms. The scope of existing solutions is extensive; we thus present the general framework and study on a case-by-case basis the relevant particularities. We describe the strategies employed to leverage the characteristics of these event-driven algorithms at the hardware level and discuss their related advantages and challenges.},
journal = {J. Emerg. Technol. Comput. Syst.},
month = {apr},
articleno = {22},
numpages = {35},
keywords = {machine learning, neuromorphic computing, hardware implementation, neural network, spiking, spiking neural networks, Neuromorphic computing, hardware, event driven}
}

@article{Fur16,
	doi = {10.1088/1741-2560/13/5/051001},
	url = {https://doi.org/10.1088/1741-2560/13/5/051001},
	year = 2016,
	month = {aug},
	publisher = {{IOP} Publishing},
	volume = {13},
	number = {5},
	pages = {051001},
	author = {Steve Furber},
	title = {Large-scale neuromorphic computing systems},
	journal = {Journal of Neural Engineering},
	abstract = {Neuromorphic computing covers a diverse range of approaches to information processing all of which demonstrate some degree of neurobiological inspiration that differentiates them from mainstream conventional computing systems. The philosophy behind neuromorphic computing has its origins in the seminal work carried out by Carver Mead at Caltech in the late 1980s. This early work influenced others to carry developments forward, and advances in VLSI technology supported steady growth in the scale and capability of neuromorphic devices. Recently, a number of large-scale neuromorphic projects have emerged, taking the approach to unprecedented scales and capabilities. These large-scale projects are associated with major new funding initiatives for brain-related research, creating a sense that the time and circumstances are right for progress in our understanding of information processing in the brain. In this review we present a brief history of neuromorphic engineering then focus on some of the principal current large-scale projects, their main features, how their approaches are complementary and distinct, their advantages and drawbacks, and highlight the sorts of capabilities that each can deliver to neural modellers.}
}

@inproceedings{CS96:DAC,
author = {Chandramouli, V. and Sakallah, Karem A.},
title = {Modeling the Effects of Temporal Proximity of Input Transitions on Gate Propagation Delay and Transition Time},
year = {1996},
isbn = {0897917790},
url = {https://doi.org/10.1145/240518.240635},
doi = {10.1145/240518.240635},
booktitle = {Proc. DAC'96},
pages = {617–622},
}


@Inbook{Hen00,
author="Henzinger, Thomas A.",
editor="Inan, M. Kemal
and Kurshan, Robert P.",
title="The Theory of Hybrid Automata",
bookTitle="Verification of Digital and Hybrid Systems",
year="2000",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="265--292",
abstract="A hybrid automaton is a formal model for a mixed discrete-continuous System. W e classify hybrid automata acoording to what questions about their behavior can be answered algorithmically. The Classification reveals structure on mixed discrete-continuous State Spaces that was previously studied on purely discrete state Spaces only. In particular, various classes of hybrid automata induce finitary trace equivalence (or similarity, or bisimilarity) relations on an uncountable State space, thus permitting the application of various model-checking techniques that were originally developed for finite state Systems.",
isbn="978-3-642-59615-5",
doi={10.1007/978-3-642-59615-5\_13},
}

@misc{FFNS23:arxiv,
      title={Continuity of Thresholded Mode-Switched ODEs and Digital Circuit Delay Models}, 
      author={Arman Ferdowsi and Matthias Függer and Thomas Nowak and Ulrich Schmid},
      year={2023},
      eprint={2303.14048},
      archivePrefix={arXiv},
      primaryClass={eess.SY},
note = {(to appear in HSCC'23)}
}

@misc{OS23:arxiv,
      title={A Digital Delay Model Supporting Large Adversarial Delay Variations}, 
      author={Daniel Öhlinger and Ulrich Schmid},
      year={2023},
      eprint={2301.09588},
      archivePrefix={arXiv},
      primaryClass={cs.OH},
note={(to appear at DDECS'23)},
}

@article{nagel1973spice,
  title={Spice (simulation program with integrated circuit emphasis)},
  author={Nagel, Laurence and Pederson, Donald O},
  year={1973}
}

@article{najm1994survey,
  title={A survey of power estimation techniques in VLSI circuits},
  author={Najm, Farid N},
  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  volume={2},
  number={4},
  pages={446--455},
  year={1994},
  publisher={IEEE}
}

==> mybib.tex <==
% Encoding: UTF-8
@techreport{NP73:spice,
    Author = {Nagel, Laurence W. and Pederson, D.O.},
    Title = {{SPICE} ({S}imulation {P}rogram with {I}ntegrated {C}ircuit {E}mphasis)},
    Institution = {EECS Department, University of California, Berkeley},
    Year = {1973},
    OPTURL = {http://www.eecs.berkeley.edu/Pubs/TechRpts/1973/22871.html},
    Number = {UCB/ERL M382}
}

@ARTICLE{DS90,
author={Deng, A.-C. and Shiau, Y.-C.},
journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
title={Generic linear {RC} delay modeling for digital {CMOS} circuits},
year={1990},
volume={9},
number={4},
pages={367--376},
OPTdoi={10.1109/43.45868},
OPTISSN={0278-0070}
}

@PhdThesis{Ho84:thesis,
  author = 	 {Mark Alan Horowitz},
  title = 	 {Timing Models for {MOS} Circuits},
  school = 	 {Stanford University},
  year = 	 {1984},
  OPTkey = 	 {},
  OPTtype = 	 {},
  OPTaddress = 	 {},
  OPTmonth = 	 {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@ARTICLE{LM84,
author={Tzu-Mu Lin and Mead, C.A.},
journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
title={Signal Delay in General {RC} Networks},
year={1984},
volume={3},
number={4},
pages={331--349},
OPTdoi={10.1109/TCAD.1984.1270090},
OPTISSN={0278-0070}
}

@ARTICLE{PR90,
author={Pillage, L.T. and Rohrer, R.A.},
journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
title={Asymptotic waveform evaluation for timing analysis},
year={1990},
volume={9},
number={4},
pages={352--366},
OPTdoi={10.1109/43.45867},
OPTISSN={0278-0070}
}

@book{Ash08,
author = {Peter J. Ashenden},
title = {The Designer’s Guide to VHDL},
edition = {third},
publisher = {Morgan Kaufmann},
address = {Burlington},
year = 2008
}

@article{BJ83,
author = {Jos\'e C. Barros and Brian W. Johnson},
title = {Equivalence of the Arbiter, the Synchronizer, the Latch, and the
Inertial Delay},
journal = {IEEE Transactions on Computers},
volume = 32,
number = 7,
pages = {603--614},
year = 1983
}

@article{BDJCAVH00,
author = {M. J. Bellido-D{\'{\i}}az
	and J. Juan-Chico
	and A. J. Acosta
	and M. Valencia
	and J. L. Huertas},
title = {Logical Modelling of Delay Degradation Effect in Static {CMOS} Gates},
journal = {IEE Proceedings -- Circuits, Devices, and Systems},
volume = 147,
number = 2,
pages = {107--117},
year = 2000
}

@article{Bra95,
author = {Michael S. Branicky},
title = {Universal Computation and Other Capabilities of Hybrid and Continuous
Dynamical Systems},
journal = {Theoretical Computer Science},
volume = 138,
number = 1,
pages = {67--100},
year = 1995
}

@article{BE92,
author = {Janusz A. Brzozowski and Jo C. Ebergen},
title = {On the Delay-Sensitivity of Gate Networks},
journal = {IEEE Transactions on Computers},
volume = 41,
number = 11,
pages = {1349--1360},
year = 1992
}

@book{Dol00,
author = {Shlomi Dolev},
title = {Self-Stabilization},
publisher = {MIT Press},
address = {Cambridge},
year = 2000
}

@incollection{DFLS11,
author = {D. Dolev and M. F\"ugger and C. Lenzen and U. Schmid},
title = {Fault-Tolerant Algorithms for Tick-Generation in Asynchronous Logic:
Robust Pulse Generation},
booktitle = {Proceeding of the 13th International Symposium on Stabilization,
Safety, and Security of Distributed Systems (SSS)},
editor = {Xavier D\'efago and Franck Petit and Vincent Villain},
series    = {LNCS},
volume    = {6976},
publisher = {Springer},
address = {Heidelberg},
pages = {163--177},
year = 2011
}


@book{DT97,
author = {Michael Drmota and Robert F. Tichy},
title = {Sequences, Discrepancies, and Applications},
publisher = {Springer},
address = {Heidelberg},
year = 1997
}

@incollection{FFS09,
author = {Gottfried Fuchs and Matthias F\"ugger and Andreas Steininger},
title = {On the Threat of Metastability in an Asynchronous Fault- Tolerant
Clock Generation Scheme},
booktitle = {Proceedings of the 15th IEEE International Symposium on
Asynchronous Circuits and Systems (ASYNC)},
publisher = {IEEE Press},
address = {New York City},
pages = {127--136},
year  =2009
}

@article{FS12,
author = {Matthias F\"ugger and Ulrich Schmid},
title = {Reconciling Fault-Tolerant Distributed Computing and Systems-on-Chip},
journal = {Distributed Computing},
volume = 14,
number = 6,
pages = {323--355},
year = 2012
}

@article{GEBC06,
author = {Matthew J. Gadledge and Paul H. Eaton and Joseph M. Benedetto and
Marty Carts and Vivian Zhu and Thomas L. Turflinger},
title = {Digital Device Error Rate Trends in Advanced {CMOS} Technologies},
journal = {IEEE Transactions on Nuclear Science},
volume = 53,
number = 6,
pages = {3466--3471},
year = 2006
}

@book{Kin07,
author = {David J. Kinniment},
title = {Synchronization and Arbitration in Digital Systems},
publisher = {Wiley},
address = {Chichester},
year = 2007
}

@article{Mar77,
author = {Leonard R. Marino},
title = {The Effect of Asynchronous Inputs on Sequential Network Reliability},
journal = {IEEE Transactions on Computers},
volume = 26,
number = 11,
pages = {1082--1090},
year = 1977
}

@article{Mar81,
author = {Leonard R. Marino},
title = {General Theory of Metastable Operation},
journal = {IEEE Transactions on Computers},
volume = 30,
number = 2,
pages = {107--115},
year = 1981
}

@incollection{MA01,
author = {M. Salim Maza and M. Linares Aranda},
title = {Analysis of Clock Distribution Networks in the Presence of Crosstalk
and Groundbounce},
booktitle = {Proceedings of the 8th IEEE International Conference on
Electronics, Circuits, and Systems (ICECS)},
publisher = {IEEE Press},
address = {New York City},
pages = {773--776},
year = 2001
}

@article{MS93,
author = {Michael Mendler and Terry Stroup},
title = {Newtonian Arbiters Cannot Be Proven Correct},
journal = {Formal Methods in System Design},
volume = 3,
number = 3,
pages = {233--257},
year = 1993
}

@article{RCS90,
author = {Fred U. Rosenberger and Charles E. Molnar and Thomas J. Chaney and
Ting-Pien Fang},
title = {Q-Modules: Internally Clocked Delay-Insensitive Modules},
journal = {IEEE Transactions on Computers},
volume = 37,
number = 9,
pages = {1005--1018},
year = 1988
}

@article{Sch93,
author = {Johannes Schoissengeier},
title = {The discrepancy of $(n\alpha)_{n\geq1}$},
journal = {Mathematische Annalen},
volume = 296,
number = 1,
pages = {529--545},
year = 1993
}

@article{Sut89,
author = {Ivan E. Sutherland},
title = {Micropipelines},
journal = {Communications of the ACM},
volume = 32,
number = 6,
pages = {720--738},
year = 1989
}

@article{Ung71,
author = {Stephen H. Unger},
title = {Asynchronous Sequential Switching Circuits with Unrestricted Input
Changes},
journal = {IEEE Transaction on Computers},
volume = 20,
number = 12,
pages = {1437--1444},
year = 1971
}

@book{BJV06,
author = {Manuel J. Bellido-D{\'{\i}}az and Jorge Juan-Chico and Manuel Valencia},
title = {Logic-Timing Simulation and
the Degradation Delay Model},
publisher = {Imperial College Press},
address = {London},
year = 2006
}

@article{Con03,
author = {Cristian Constantinescu},
title = {Trends and Challenges in {VLSI} Circuit Reliability},
journal = {IEEE Micro},
volume = 23,
number = 4,
pages = {14--19},
year = 2003
}

@incollection{FNS13,
author = {Matthias F\"ugger and Thomas Nowak and Ulrich Schmid},
title = {Unfaithful Glitch Propagation in Existing Binary Circuit Models},
booktitle = {Proceedings of the 19th IEEE International Symposium on
Asynchronous Circuits and Systems (ASYNC)},
publisher = {IEEE Press},
address = {New York City},
pages = {191--199},
year = 2013
}

@MISC{Syn05:CCS,
author={Synopsis},
title={{CCS} Timing},
howpublished={Technical white paper v2.0, 2006},
}


@ARTICLE{Naj94,
author={Najm, F.N.},
journal={Very Large Scale Integration (VLSI) Systems, IEEE Transactions on},
title={A survey of power estimation techniques in {VLSI} circuits},
year={1994},
volume={2},
number={4},
pages={446-455},
doi={10.1109/92.335013},
ISSN={1063-8210}
}
@inproceedings{FB95,
 author = {Favalli, M. and Benini, L.},
 title = {Analysis of glitch power dissipation in {CMOS} {IC}s},
 booktitle = {Proceedings of the 1995 international symposium on Low power desig
n},
 series = {ISLPED '95},
 year = {1995},
 isbn = {0-89791-744-8},
 location = {Dana Point, California, USA},
 pages = {123--128},
 numpages = {6},
 doi = {10.1145/224081.224103},
 acmid = {224103},
 publisher = {ACM},
 address = {New York, NY, USA},
}
@inproceedings{FNS13:ASYNC,
  author    = {Matthias F{\"u}gger and Thomas Nowak and Ulrich Schmid},
  title     = {Unfaithful Glitch Propagation in Existing Binary Circuit Models},
  booktitle = {Proceedings 19th IEEE International Symposium on Asynchronous Circuits and Systems (ASYNC'13)},
  year      = {2013},
  pages = {191-199},
ee        = {http://doi.ieeecomputersociety.org/10.1109/ASYNC.2013.9},
publisher = {IEEE Computer Society},
}

@ARTICLE{FNS16:ToC,
author={Matthias F\"ugger and Thomas Nowak and Ulrich Schmid},
journal={IEEE Transactions on Computers},
title={Unfaithful Glitch Propagation in Existing Binary Circuit Models},
year={2016},
volume={65},
number={3},
pages={964-978},
keywords={Analytical models;Computational modeling;Delays;Integrated circuit mod
eling;Inverters;Logic gates;Circuit models;binary models;glitch propagation;mode
ling issues},
doi={10.1109/TC.2015.2435791},
ISSN={0018-9340},
month={March},
}

@incollection{JBRA00,
year={2000},
isbn={978-3-540-41068-3},
booktitle={Integrated Circuit Design},
series={LNCS 1918},
doi={10.1007/3-540-45373-3_15},
title={Degradation Delay Model Extension to {CMOS} Gates},
publisher={Springer},
author={Juan-Chico, Jorge and Bellido, Manuel J. and Ruiz-de-Clavijo, Paulino and Acosta, Antonio J. and Valencia, Manuel},
pages={149-158},
language={English}
}

@incollection{MJBR02,
year={2002},
isbn={978-3-540-44143-4},
booktitle={Integrated Circuit Design},
series={LNCS 2451},
doi={10.1007/3-540-45716-X_48},
title={Characterization of Normal Propagation Delay for Delay Degradation Model {(DDM)}},
publisher={Springer},
author={Millan, Alejandro and Juan, Jorge and Bellido, Manuel J. and Ruiz-de-Clavijo, Paulino and Guerrero, David},
pages={477-486},
language={English}
}

@article{HSDZ12:ToNS,
  author =       "Michael Hofbauer and Kurt Schweiger and Horst Dietrich and Horst Zimmermann and Kay-Obbe Voss and Bruno Merk and Ulrich Schmid and Andreas Steininger",
  title =        "Pulse Shape Measurements by On-chip Sense Amplifiers of Single
 Event Transients Propagating through a 90 nm Bulk {CMOS} Inverter Chain",
  journal =      "IEEE Transactions on Nuclear Science",
  year =         "2012",
  month = dec,
  volume = 59,
  number = 6,
  pages = {2778-2784},
}

@manual{Syn:CCSM,
organization={Synopsis Inc.},
title={{CCS} Timing Library Characterization Guidelines},
month={October},
year={2016},
note={Version 3.4}
}

@manual{Cad:ECSM,
organization={Cadence Design Systems},
title={Effective Current Source Model {(ECSM)} Timing and Power Specification},
month={January},
year={2015},
note={Version 2.1.2}
}

@inproceedings{NFNS15:GLSVLSI,
 author = {Najvirt, Robert and Schmid, Ulrich and Hofbauer, Michael and F\"{u}gger, Matthias and Nowak, Thomas and Schweiger, Kurt},
 title = {Experimental Validation of a Faithful Binary Circuit Model},
 booktitle = {Proceedings of the 25th Edition on Great Lakes Symposium on VLSI},
 series = {GLSVLSI '15},
 year = {2015},
 isbn = {978-1-4503-3474-7},
 location = {Pittsburgh, Pennsylvania, USA},
 pages = {355--360},
 numpages = {6},
 url = {http://doi.acm.org/10.1145/2742060.2742081},
 doi = {10.1145/2742060.2742081},
 acmid = {2742081},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {binary circuit models, delay models, vlsi},
} 


@book{BJV:DDM05,
author = {Bellido, Manuel J and Juan, Jorge and Valencia, Manuel},
title = {Logic-Timing Simulation and the Degradation Delay Model},
publisher = {Imperial College},
year = {2005},
doi = {10.1142/p411},
address = {},
edition   = {},
URL = {https://www.worldscientific.com/doi/abs/10.1142/p411},
eprint = {https://www.worldscientific.com/doi/pdf/10.1142/p411}
}

@inproceedings{FNNS15:DATE,
 author = {F\"{u}gger, Matthias and Najvirt, Robert and Nowak, Thomas and Schmid, Ulrich},
 title = {Towards Binary Circuit Models That Faithfully Capture Physical Solvability},
 booktitle = {Proceedings of the 2015 Design, Automation \& Test in Europe Conference \& Exhibition},
 series = {DATE '15},
 year = {2015},
 pages = {1455--1460},
 publisher = {EDA Consortium},
 address = {San Jose, CA, USA},
}

@INPROCEEDINGS{FMNNS18:DATE,
author={M. F{\"u}gger and J. Maier and R. Najvirt and T. Nowak and U. Schmid},
booktitle={2018 Design, Automation Test in Europe Conference Exhibition (DATE)},
title={A faithful binary circuit model with adversarial noise},
year={2018},
volume={},
number={},
pages={1327-1332},
keywords={delay circuits;digital circuits;formal verification;network synthesis;IEEE TC 2016;accurate delay models;adversarial noise;delay functions;delay shifts;deterministic delay function;digital circuits;dynamic timing analysis;even adversarial;faithful binary circuit model;faithful digital circuit models;formal verification;generalized involution model;involution delays;mathematical involutions;nondeterministic delay variations;pure inertial delays;random adversarial;static timing analysis;Analytical models;Delays;Digital circuits;Integrated circuit modeling;Logic gates;Tools},
doi={10.23919/DATE.2018.8342219},
ISSN={},
month={March},
url={https://ieeexplore.ieee.org/document/8342219/}
}

@BOOK{arora1993,
author = {Arora, Narain},
title = {MOSFET models for VLSI circuit simulation; theory and practice},
series = {Computational microelectronics},
year = {1993},
address = {Wien [u.a.]},
publisher = {Springer},
ISBN = {3-211-82395-6; 0-387-82395-6},
keywords = {MOS-FET ; VLSI; Freies Schlagwort: MOS-FET - VLSI; Metal oxide
semiconductor field-effect transistors ; Mathematical models; Integrated
circuits ; Very large scale integration ; Mathematical models; Integrated
circuits ; Very large scale integration ; Computer simulation},
}

@techreport{M17:TR,
key = {2017},
    author = {Maier, J{\"u}rgen},
    title = {Modeling the CMOS Inverter using Hybrid Systems},
    institution = {E182 - Institut f{\"u}r Technische Informatik; Technische Universit{\"a}t Wien},
    year = {2017},
    number = {TUW-259633},
    url = {http://publik.tuwien.ac.at/files/publik\_259633.pdf}
}

@book {Sze,
title = {Physics of Semiconductor Devices},
author = {Sze, S.M. and Ng, Kwok K.},
publisher = {John Wiley \& Sons, Inc.},
isbn = {9780471143239},
year = {2007},
edition = {third}
}

@MISC{Mathematica,
title={Wolfram Mathematica},
howpublished={\url{https://www.wolfram.com/mathematica/}},
note={Accessed: 2018-12-07}
}


@INPROCEEDINGS{JBAB93,
    author = {Juan-Chico Bellido Acosta and J. Juan-chico and M. J. Bellido and A. J. Acosta and A. Bar
riga and M. Valencia and Sevilla Centro and Nacional Microelectrónica},
    title = {Delay degradation effect in submicronic {CMOS} inverters},
    booktitle = {Proc. FODO'93},
    year = {1997},
    pages = {215--224},
    publisher = {Springer}
}

@inproceedings{Nangate15,
 author = {Martins, Mayler and Matos, Jody Maick and Ribas, Renato P. and Reis, Andr{\'e} and Schlinker, Guilherme and Rech, Lucio and Michelsen, Jens},
 title = {Open Cell Library in 15Nm FreePDK Technology},
 booktitle = {Proceedings of the 2015 Symposium on International Symposium on Physical Design},
 series = {ISPD '15},
 year = {2015},
 isbn = {978-1-4503-3399-3},
 location = {Monterey, California, USA},
 pages = {171--178},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/2717764.2717783},
 doi = {10.1145/2717764.2717783},
 acmid = {2717783},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@INPROCEEDINGS{CharlieEffect,
author={A. J. Winstanley and A. Garivier and M. R. Greenstreet},
booktitle={Proceedings of the 8th International Symposium on Asynchronous Circuits and Systems (ASYNC)},
title={{An Event Spacing Experiment}},
year={2002},
pages={47-56},
keywords={asynchronous circuits;delays;hysteresis;pipeline
processing;timing;Charlie Diagrams;attractors;evenly spaced behaviours;event
spacing experiment;hysteresis;phase transitions;self-timed pipelines;self-timed
rings;standard bounded delay models;timing analysis;Clocks;Delay;Distributed
processing;Fabrication;Hysteresis;Pipelines;Semiconductor device
modeling;Testing;Throughput;Timing}, 
doi={10.1109/ASYNC.2002.1000295},
ISSN={1522-8681},
month={April},}

@book{strang2014differential,
  title={Differential equations and linear algebra},
  author={Strang, Gilbert},
  year={2014},
  publisher={Wellesley-Cambridge Press Wellesley}
}

@INPROCEEDINGS{EFS98:ASYNC,
  author={J. C. {Ebergen} and S. {Fairbanks} and I. E. {Sutherland}},
  booktitle={Proceedings Fourth International Symposium on Advanced Research in Asynchronous Circuits and Systems (ASYNC'98)}, 
  title={Predicting performance of micropipelines using Charlie diagrams}, 
  year={1998},
  volume={},
  number={},
  pages={238-246},
  doi={10.1109/ASYNC.1998.666509}}

@ARTICLE{FNNS19:TCAD,
author={M. {Függer} and R. {Najvirt} and T. {Nowak} and U. {Schmid}},
journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
title={A Faithful Binary Circuit Model},
year={2020},
volume={39},
number={10},
pages={2784-2797},
keywords={Binary circuit models;glitch propagation},
doi={10.1109/TCAD.2019.2937748},
ISSN={0278-0070},}
%month={October},}

@article{OMFS20:INTEGRATION,
title = "The Involution Tool for Accurate Digital Timing and Power Analysis",
journal = "Integration",
volume = "76",
pages = "87 - 98",
year = "2021",
issn = "0167-9260",
doi = "https://doi.org/10.1016/j.vlsi.2020.09.007",
author = "Daniel Öhlinger and Jürgen Maier and Matthias Függer and Ulrich Schmid",
keywords = "Digital timing simulation, Design tools, Delay models, Pulse degradation, Glitch propagation",
}

@Manual{MSIM:FLI,
  title  = {Foreign Language Interface Manual},
  author = {{Mentor Graphics Corporation}},
  note   = {{Software Version 10.5c}},
  year   = {2016},
}

@INPROCEEDINGS{CGB01:DAC,
author={Liang-Chi Chen and S. K. Gupta and M. A. Breuer},
booktitle={Proceedings of the 38th Design Automation Conference (IEEE
Cat. No.01CH37232)}, 
title={A new gate delay model for simultaneous switching and its applications},
year={2001},
pages={289-294},
keywords={automatic test pattern generation;combinational circuits;delays;logic
gates;logic testing;timing;delay phenomena;gate delay model;incremental timing
refinement;simultaneous switching;static timing analysis;targeted delay
phenomena;timing-based ATPG;to-controlling transitions;transition
times;Accuracy;Automatic test pattern generation;Benchmark
testing;Circuits;Computational modeling;Delay effects;Performance
analysis;Permission;Table lookup;Timing}, 
doi={10.1109/DAC.2001.156153},
ISSN={0738-100X},
month={},}

@article{SRC15:TDAE,
 author = {Subramaniam, Anupama R. and Roveda, Janet and Cao, Yu},
 title = {A Finite-Point Method for Efficient Gate Characterization Under
 Multiple Input Switching},
 journal = {ACM Trans. Des. Autom. Electron. Syst.},
 issue_date = {November 2015},
 volume = {21},
 number = {1},
 month = dec,
 year = {2015},
 issn = {1084-4309},
 pages = {10:1--10:25},
 articleno = {10},
 numpages = {25},
 url = {http://doi.acm.org/10.1145/2778970},
 doi = {10.1145/2778970},
 acmid = {2778970},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Characterization, design flow, finite point method, flow, logic,
 multiple input switching, performance verification, standard cell
 characterization}, 
} 


@INPROCEEDINGS{SKJPC09:ISOCC,
author={J. Shin and J. Kim and N. Jang and E. Park and Y. Choi},
booktitle={2009 International SoC Design Conference (ISOCC)},
title={A gate delay model considering temporal proximity of Multiple Input
Switching}, 
year={2009},
pages={577-580},
keywords={delay circuits;integrated circuit modelling;radial basis function
networks;accurate gate delay;delay variation;gate delay model;multiple input
switching;radial basis function;temporal proximity;Capacitance;Circuit
analysis;Clocks;Computer science;Delay effects;Delay
estimation;Frequency;Libraries;MOSFETs;Timing;cell characterization;delay
model;multiple input switching;proximity;temporal}, 
doi={10.1109/SOCDC.2009.5423815},
month={Nov},}

@INPROCEEDINGS{SC06:DATE,
author={J. Sridharan and T. Chen},
booktitle={Proceedings of the Design Automation Test in Europe Conference},
title={Modeling multiple input switching of CMOS gates in DSM technology using
HDMR}, 
year={2006},
volume={1},
pages={6 pp.-},
keywords={CMOS logic circuits;delays;integrated circuit modelling;logic
gates;CMOS gates;DSM chips;SPICE;gate level delays;high dimensional model
representation method;logic gate;multiple input switching modeling;relative
signal arrival times;static timing analysis;CMOS logic circuits;CMOS
technology;Clocks;Delay effects;Delay systems;Logic gates;Semiconductor device
modeling;Signal analysis;Signal processing;Timing}, 
doi={10.1109/DATE.2006.244008},
ISSN={1530-1591},
month={March},}

@ARTICLE{RS21:TCAD,
  author={Shashank Ram, O. V. S. and Saurabh, Sneh},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems}, 
  title={Modeling Multiple-Input Switching in Timing Analysis Using Machine Learning}, 
  year={2021},
  volume={40},
  number={4},
  pages={723-734},
  doi={10.1109/TCAD.2020.3009624}}

@article{Melcher92:MAM,
title = "Multiple input transitions in CMOS gates",
journal = "Microprocessing and Microprogramming",
volume = "35",
number = "1",
pages = "683 - 690",
year = "1992",
note = "Software and Hardware: Specification and Design",
issn = "0165-6074",
doi = "http://dx.doi.org/10.1016/0165-6074(92)90387-M",
url = "http://www.sciencedirect.com/science/article/pii/016560749290387M",
author = "Elmar Melcher and Wolfgang Röthig and Michel Dana",
}

@INPROCEEDINGS{AB06:SST,
author={N. Abdallah and P. Bazargan-Sabet},
booktitle={2006 Proceeding of the Thirty-Eighth Southeastern Symposium on System Theory},
title={Modeling the Effects of Input Slew Rate and Temporal Proximity of Input
Transitions in Event-Driven Simulation}, 
year={2006},
pages={185-189},
keywords={MOS digital integrated circuits;circuit simulation;MOS digital
circuits;event-driven selective-trace paradigm;input slew rate;input
transitions;switch-level timing simulation;temporal proximity;Accuracy;Circuit
simulation;Digital circuits;Discrete event simulation;Predictive
models;Shape;Switching circuits;Timing;Very large scale integration;Voltage}, 
doi={10.1109/SSST.2006.1619069},
ISSN={0094-2898},
month={March},}

@INPROCEEDINGS{SHWW14:ICCAD,
  author={Schneider, Eric and Holst, Stefan and Wen, Xiaoqing and Wunderlich, Hans-Joachim},
  booktitle={2014 IEEE/ACM International Conference on Computer-Aided Design (ICCAD)}, 
  title={Data-parallel simulation for fast and accurate timing validation of CMOS circuits}, 
  year={2014},
  volume={},
  number={},
  pages={17-23},
  doi={10.1109/ICCAD.2014.7001324}}


@inproceedings{FMOS22:DATE,
  author    = {Arman Ferdowsi and
               J{\"{u}}rgen Maier and
               Daniel {\"{O}}hlinger and
               Ulrich Schmid},
  title     = {A Simple Hybrid Model for Accurate Delay Modeling of a Multi-Inpu
t
               Gate},
booktitle = {Proceedings of the 2022 Design, Automation \& Test in Europe Confer
ence \& Exhibition},
 series = {DATE '22},
  year      = {2022},
}


@misc{FMOS21:arxiv,
      title={{A Simply Hybrid Model for Accurate Delay Modeling of a Multi-Input Gate}},
      author={Arman Ferdowsi and J\"urgen Maier and Daniel \"Ohlinger and Ulrich Schmid},
      year={2021},
      note={TechRxiv e-prints, to appear in Proc. DATE'22},
      doi={10.36227/techrxiv.17054906},
      url = {http://doi.acm.org/10.36227/techrxiv.17054906},
}

@ARTICLE{ShichmanHodges,
author={H. {Shichman} and D. A. {Hodges}},
journal={IEEE Journal of Solid-State Circuits},
title={Modeling and simulation of insulated-gate field-effect transistor switching circuits},
year={1968},
volume={3},
number={3},
pages={285-289},
keywords={computer-aided circuit analysis;Computer-aided circuit
                  analysis;Circuit simulation;Insulation;FETs;Switching
                  circuits;Computational modeling;Equivalent circuits;Computer
                  aided analysis;Computer simulation;Application
                  software;Application specific integrated circuits},
doi={10.1109/JSSC.1968.1049902},
ISSN={0018-9200},
month={Sep.},}


@Comment{jabref-meta: databaseType:bibtex;}

%url = "http://www.sciencedirect.com/science/article/pii/S0167926020302777",

@article{BVMRRVB19,
author = {Bouvier, Maxence and Valentian, Alexandre and Mesquida, Thomas and Rummens, Francois and Reyboz, Marina and Vianello, Elisa and Beigne, Edith},
title = {Spiking Neural Networks Hardware Implementations and Challenges: A Survey},
year = {2019},
issue_date = {April 2019},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {15},
number = {2},
issn = {1550-4832},
url = {https://doi.org/10.1145/3304103},
doi = {10.1145/3304103},
abstract = {Neuromorphic computing is henceforth a major research field for both academic and industrial actors. As opposed to Von Neumann machines, brain-inspired processors aim at bringing closer the memory and the computational elements to efficiently evaluate machine learning algorithms. Recently, spiking neural networks, a generation of cognitive algorithms employing computational primitives mimicking neuron and synapse operational principles, have become an important part of deep learning. They are expected to improve the computational performance and efficiency of neural networks, but they are best suited for hardware able to support their temporal dynamics. In this survey, we present the state of the art of hardware implementations of spiking neural networks and the current trends in algorithm elaboration from model selection to training mechanisms. The scope of existing solutions is extensive; we thus present the general framework and study on a case-by-case basis the relevant particularities. We describe the strategies employed to leverage the characteristics of these event-driven algorithms at the hardware level and discuss their related advantages and challenges.},
journal = {J. Emerg. Technol. Comput. Syst.},
month = {apr},
articleno = {22},
numpages = {35},
keywords = {machine learning, neuromorphic computing, hardware implementation, neural network, spiking, spiking neural networks, Neuromorphic computing, hardware, event driven}
}

@article{Fur16,
	doi = {10.1088/1741-2560/13/5/051001},
	url = {https://doi.org/10.1088/1741-2560/13/5/051001},
	year = 2016,
	month = {aug},
	publisher = {{IOP} Publishing},
	volume = {13},
	number = {5},
	pages = {051001},
	author = {Steve Furber},
	title = {Large-scale neuromorphic computing systems},
	journal = {Journal of Neural Engineering},
	abstract = {Neuromorphic computing covers a diverse range of approaches to information processing all of which demonstrate some degree of neurobiological inspiration that differentiates them from mainstream conventional computing systems. The philosophy behind neuromorphic computing has its origins in the seminal work carried out by Carver Mead at Caltech in the late 1980s. This early work influenced others to carry developments forward, and advances in VLSI technology supported steady growth in the scale and capability of neuromorphic devices. Recently, a number of large-scale neuromorphic projects have emerged, taking the approach to unprecedented scales and capabilities. These large-scale projects are associated with major new funding initiatives for brain-related research, creating a sense that the time and circumstances are right for progress in our understanding of information processing in the brain. In this review we present a brief history of neuromorphic engineering then focus on some of the principal current large-scale projects, their main features, how their approaches are complementary and distinct, their advantages and drawbacks, and highlight the sorts of capabilities that each can deliver to neural modellers.}
}

@inproceedings{CS96:DAC,
author = {Chandramouli, V. and Sakallah, Karem A.},
title = {Modeling the Effects of Temporal Proximity of Input Transitions on Gate Propagation Delay and Transition Time},
year = {1996},
isbn = {0897917790},
url = {https://doi.org/10.1145/240518.240635},
doi = {10.1145/240518.240635},
booktitle = {Proc. DAC'96},
pages = {617–622},
}


@Inbook{Hen00,
author="Henzinger, Thomas A.",
editor="Inan, M. Kemal
and Kurshan, Robert P.",
title="The Theory of Hybrid Automata",
bookTitle="Verification of Digital and Hybrid Systems",
year="2000",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="265--292",
abstract="A hybrid automaton is a formal model for a mixed discrete-continuous System. W e classify hybrid automata acoording to what questions about their behavior can be answered algorithmically. The Classification reveals structure on mixed discrete-continuous State Spaces that was previously studied on purely discrete state Spaces only. In particular, various classes of hybrid automata induce finitary trace equivalence (or similarity, or bisimilarity) relations on an uncountable State space, thus permitting the application of various model-checking techniques that were originally developed for finite state Systems.",
isbn="978-3-642-59615-5",
doi={10.1007/978-3-642-59615-5\_13},
}

@misc{FFNS23:arxiv,
      title={Continuity of Thresholded Mode-Switched ODEs and Digital Circuit Delay Models}, 
      author={Arman Ferdowsi and Matthias Függer and Thomas Nowak and Ulrich Schmid},
      year={2023},
      eprint={2303.14048},
      archivePrefix={arXiv},
      primaryClass={eess.SY},
note = {(to appear in HSCC'23)}
}

@misc{OS23:arxiv,
      title={A Digital Delay Model Supporting Large Adversarial Delay Variations}, 
      author={Daniel Öhlinger and Ulrich Schmid},
      year={2023},
      eprint={2301.09588},
      archivePrefix={arXiv},
      primaryClass={cs.OH},
note={(to appear at DDECS'23)},
}

@article{nagel1973spice,
  title={Spice (simulation program with integrated circuit emphasis)},
  author={Nagel, Laurence and Pederson, Donald O},
  year={1973}
}

@article{najm1994survey,
  title={A survey of power estimation techniques in VLSI circuits},
  author={Najm, Farid N},
  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  volume={2},
  number={4},
  pages={446--455},
  year={1994},
  publisher={IEEE}
}
